Low-rank Matrix Optimization Using Polynomial-filtered Subspace Extraction

In this paper, we study first-order methods on a large variety of low-rank matrix optimization problems, whose solutions only live in a low dimensional eigenspace. Traditional first-order methods depend on the eigenvalue decomposition at each iteration which takes most of the computation time. In order to reduce the cost, we propose an inexact algorithm framework based on a polynomial subspace extraction. The idea is to use an additional polynomial-filtered iteration to extract an approximated eigenspace, and project the iteration matrix on this subspace, followed by an optimization update. The accuracy of the extracted subspace can be controlled by the degree of the polynomial filters. This kind of subspace extraction also enjoys the warm start property: the subspace of the current iteration is refined from the previous one. Then this framework is instantiated into two algorithms: the polynomial-filtered proximal gradient method and the polynomial-filtered alternating direction method of multipliers. We give a theoretical guarantee to the two algorithms that the polynomial degree is not necessarily very large. They share the same convergence speed as the corresponding original methods if the polynomial degree grows with an order $\Omega(\log k)$ at the $k$-th iteration. If the warm-start property is considered, the degree can be reduced to a constant, independent of the iteration $k$. Preliminary numerical experiments on several low-rank matrix optimization problems show that the polynomial filtered algorithms usually provide multi-fold speedups.

==> tab/G.tex <==
G22 & 2000 & 1.413595e+04 &   0.57 &    248 & 9.5e-15 & 1.413648e+04 & 2.54 && 68  \\ 
G23 & 2000 & 1.414551e+04 &   0.64 &    313 & 9.7e-15 & 1.414644e+04 & 3.42 && 138 \\ 
G24 & 2000 & 1.414086e+04 &   0.47 &    247 & 9.7e-15 & 1.414154e+04 & 3.03 && 113 \\ 
G25 & 2000 & 1.414425e+04 &   0.42 &    213 & 9.5e-15 & 1.414478e+04 & 2.94 && 105 \\ 
G26 & 2000 & 1.413287e+04 &   0.43 &    215 & 9.4e-15 & 1.413330e+04 & 2.98 && 113 \\ 
G27 & 2000 & 4.141659e+03 &   0.49 &    239 & 9.7e-15 & 4.142276e+03 & 2.71 && 91  \\ 
G28 & 2000 & 4.100790e+03 &   0.65 &    311 & 9.5e-15 & 4.101243e+03 & 2.85 && 99  \\ 
G29 & 2000 & 4.208889e+03 &   0.49 &    223 & 9.2e-15 & 4.209374e+03 & 2.36 && 76  \\ 
G30 & 2000 & 4.215382e+03 &   0.44 &    207 & 9.4e-15 & 4.216098e+03 & 2.04 && 69  \\ 
G31 & 2000 & 4.116682e+03 &   0.46 &    222 & 9.5e-15 & 4.116912e+03 & 3.19 && 121 \\ 
G32 & 2000 & 1.567634e+03 &   1.14 &   1034 & 9.8e-15 & 1.567784e+03 & 15.74 && 927 \\ 
G33 & 2000 & 1.544310e+03 &   1.10 &   1021 & 9.1e-15 & 1.544377e+03 & 19.07 && 1141\\ 
G34 & 2000 & 1.546686e+03 &   0.70 &    657 & 9.2e-15 & 1.546802e+03 & 13.62 && 805 \\ 
G35 & 2000 & 8.014736e+03 &   0.60 &    404 & 9.5e-15 & 8.015651e+03 & 5.42 && 212  \\ 
G36 & 2000 & 8.005956e+03 &   0.74 &    540 & 9.6e-15 & 8.007743e+03 & 4.21 && 177  \\ 
G37 & 2000 & 8.018617e+03 &   0.76 &    562 & 9.7e-15 & 8.019592e+03 & 4.61 && 197  \\ 
G38 & 2000 & 8.014970e+03 &   0.64 &    492 & 9.5e-15 & 8.016159e+03 & 3.22 && 107  \\ 
G39 & 2000 & 2.877644e+03 &   0.45 &    348 & 9.7e-15 & 2.879072e+03 & 4.84 && 242  \\ 
G40 & 2000 & 2.864786e+03 &   0.55 &    430 & 9.6e-15 & 2.872892e+03 & 5.56 && 266  \\ 
G41 & 2000 & 2.865217e+03 &   0.63 &    409 & 9.3e-15 & 2.865422e+03 & 17.56 && 1050\\ 
G42 & 2000 & 2.946250e+03 &   0.44 &    336 & 9.5e-15 & 2.946930e+03 & 5.09 && 257  \\ 
G48 & 3000 & 6.000000e+03 &   0.40 &    258 & 1.1e-14 & 6.000000e+03 & 1.16 && 20  \\ 
G49 & 3000 & 6.000000e+03 &   0.53 &    335 & 1.1e-14 & 6.000001e+03 & 1.19 && 24  \\ 
G50 & 3000 & 5.988172e+03 &   0.49 &    323 & 1.0e-14 & 5.988176e+03 & 2.40 && 100  \\ 
G55 & 5000 & 1.103946e+04 &   1.42 &    320 & 1.5e-14 &&&& \\
G57 & 5000 & 3.885477e+03 &   3.01 &   1041 & 1.5e-14  &&&& \\
G58 & 5000 & 2.013576e+04 &   4.02 &   1028 & 1.5e-14 &&&& \\
G60 & 7000 & 1.522224e+04 &   3.21 &    562 & 1.8e-14  &&&& \\
G62 & 7000 & 5.430873e+03 &   3.18 &   1042 & 1.7e-14 &&&& \\
G63 & 7000 & 2.824292e+04 &   6.13 &   1039 & 1.8e-14&&&&  \\ 
G64 & 7000 & 1.046581e+04 &   3.15 &    760 & 1.8e-14&&&&  \\ 
G65 & 8000 & 6.205477e+03 &   5.32 &   1048 & 1.9e-14 &&&&   \\ 
G66 & 9000 & 7.077168e+03 &   5.97 &   1036 & 2.0e-14 &&&&  \\ 
G67 & 10000 &7.744367e+03 &   6.06 &   1046 & 2.2e-14 &&&&\\ 
G70 & 10000 &9.861523e+03 &   3.26 &    794 & 2.1e-14 &&&&\\ 
G72 & 10000 &7.808479e+03 &   4.61 &   1039 & 2.1e-14 &&&&\\ 
G77 & 14000 &1.104553e+04 &   7.75 &   1040 & 2.4e-14 &&&&\\ 
G81 & 20000 &1.565603e+04 &  10.00 &   1037 & 3.0e-14 &&&&\\ 


==> tab/G.tex.1 <==
G01 & 1.208404e+04 & 0.79 & 44  \\ 
G02 & 1.209016e+04 & 1.04 & 62  \\ 
G03 & 1.208483e+04 & 0.94 & 49  \\ 
G04 & 1.211209e+04 & 0.98 & 58  \\ 
G05 & 1.210296e+04 & 1.26 & 79  \\ 
G06 & 2.656260e+03 & 1.51 & 102  \\ 
G07 & 2.489323e+03 & 1.41 & 93  \\ 
G08 & 2.507146e+03 & 0.86 & 51  \\ 
G09 & 2.528883e+03 & 1.50 & 104  \\ 
G10 & 2.485137e+03 & 1.19 & 66  \\ 
G11 & 6.293623e+02 & 4.67 & 631  \\ 
G12 & 6.239483e+02 & 5.69 & 889  \\ 
G13 & 6.472341e+02 & 5.14 & 739  \\ 
G14 & 3.191971e+03 & 1.64 & 130  \\ 
G15 & 3.171801e+03 & 1.24 & 86  \\ 
G16 & 3.175132e+03 & 1.78 & 147  \\ 
G17 & 3.171656e+03 & 1.20 & 83  \\ 
G18 & 1.166090e+03 & 4.78 & 570  \\ 
G19 & 1.082131e+03 & 13.00 & 1685  \\ 
G20 & 1.111496e+03 & 3.45 & 379  \\ 
G21 & 1.104801e+03 & 1.86 & 134  \\ 
G22 & 1.413648e+04 & 2.54 & 68  \\ 
G23 & 1.414644e+04 & 3.42 & 138  \\ 
G24 & 1.414154e+04 & 3.03 & 113  \\ 
G25 & 1.414478e+04 & 2.94 & 105  \\ 
G26 & 1.413330e+04 & 2.98 & 113  \\ 
G27 & 4.142276e+03 & 2.71 & 91  \\ 
G28 & 4.101243e+03 & 2.85 & 99  \\ 
G29 & 4.209374e+03 & 2.36 & 76  \\ 
G30 & 4.216098e+03 & 2.04 & 69  \\ 
G31 & 4.116912e+03 & 3.19 & 121  \\ 
G32 & 1.567784e+03 & 15.74 & 927  \\ 
G33 & 1.544377e+03 & 19.07 & 1141  \\ 
G34 & 1.546802e+03 & 13.62 & 805  \\ 
G35 & 8.015651e+03 & 5.42 & 212  \\ 
G36 & 8.007743e+03 & 4.21 & 177  \\ 
G37 & 8.019592e+03 & 4.61 & 197  \\ 
G38 & 8.016159e+03 & 3.22 & 107  \\ 
G39 & 2.879072e+03 & 4.84 & 242  \\ 
G40 & 2.872892e+03 & 5.56 & 266  \\ 
G41 & 2.865422e+03 & 17.56 & 1050  \\ 
G42 & 2.946930e+03 & 5.09 & 257  \\ 
G43 & 7.032504e+03 & 0.77 & 49  \\ 
G44 & 7.028198e+03 & 0.93 & 56  \\ 
G45 & 7.025249e+03 & 0.97 & 56  \\ 
G46 & 7.030293e+03 & 0.83 & 48  \\ 
G47 & 7.036782e+03 & 1.33 & 103  \\ 
G48 & 6.000000e+03 & 1.16 & 20  \\ 
G49 & 6.000001e+03 & 1.19 & 24  \\ 
G50 & 5.988176e+03 & 2.40 & 100  \\ 
G51 & 4.006325e+03 & 3.65 & 338  \\ 
G52 & 4.010063e+03 & 1.94 & 143  \\ 
G53 & 4.009854e+03 & 2.51 & 205  \\ 
G54 & 4.006623e+03 & 1.47 & 86  \\ 


==> tab/Test_5_5.tex <==
\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{GBB} & \multicolumn{5}{c|}{IGBB} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 0.9   & 43 & 44 & 1.1e+05 & 4.6e-06 & 0.4  & 47 & 48 & 1.1e+05 & 9.9e-06 \\
1000 & 3.6   & 43 & 44 & 3.1e+05 & 6.9e-06 & 1.6  & 54 & 55 & 3.1e+05 & 4.6e-06 \\
1500 & 9.4   & 43 & 44 & 5.9e+05 & 9.2e-06 & 3.6  & 56 & 57 & 5.9e+05 & 9.9e-06 \\
2000 & 19.0  & 50 & 51 & 9.2e+05 & 9.9e-06 & 5.6  & 65 & 66 & 9.2e+05 & 3.7e-06 \\
2500 & 37.4  & 54 & 55 & 1.2e+06 & 1.0e-06 & 9.8  & 65 & 66 & 1.2e+06 & 4.1e-06 \\
3000 & 64.3  & 54 & 55 & 1.7e+06 & 1.1e-06 & 16.0 & 65 & 66 & 1.7e+06 & 5.2e-06 \\
4000 & 155.2 & 54 & 55 & 2.6e+06 & 1.3e-06 & 35.3 & 76 & 77 & 2.6e+06 & 4.2e-06 \\ \hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{ILBFGS} & \multicolumn{5}{c|}{Newton} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 0.3  & 21 & 22 & 1.1e+05 & 6.0e-06 & 0.5  & 8 & 9 & 1.1e+05 & 2.1e-06 \\
1000 & 1.0  & 21 & 22 & 3.1e+05 & 1.1e-05 & 1.3  & 8 & 9 & 3.1e+05 & 3.0e-06 \\
1500 & 2.7  & 24 & 25 & 5.9e+05 & 8.7e-06 & 3.3  & 8 & 9 & 5.9e+05 & 3.7e-06 \\
2000 & 4.2  & 22 & 24 & 9.2e+05 & 1.2e-05 & 6.0  & 8 & 9 & 9.2e+05 & 4.3e-06 \\
2500 & 7.2  & 22 & 25 & 1.2e+06 & 1.1e-05 & 10.0 & 8 & 9 & 1.2e+06 & 4.8e-06 \\
3000 & 12.0 & 25 & 26 & 1.7e+06 & 9.1e-06 & 16.7 & 8 & 9 & 1.7e+06 & 5.3e-06 \\
4000 & 31.1 & 25 & 26 & 2.6e+06 & 8.0e-06 & 36.2 & 8 & 9 & 2.6e+06 & 6.1e-06 \\ \hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{QN} & \multicolumn{5}{c|}{IQN} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 0.5  & 14 & 15 & 1.1e+05 & 2.0e-06 & 0.5  & 14 & 15 & 1.1e+05 & 2.0e-06 \\
1000 & 1.5  & 14 & 15 & 3.1e+05 & 2.8e-06 & 1.2  & 15 & 16 & 3.1e+05 & 2.9e-06 \\
1500 & 3.7  & 14 & 15 & 5.9e+05 & 3.8e-06 & 2.5  & 15 & 16 & 5.9e+05 & 3.6e-06 \\
2000 & 6.4  & 14 & 15 & 9.2e+05 & 4.3e-06 & 4.4  & 15 & 16 & 9.2e+05 & 4.3e-06 \\
2500 & 11.5 & 14 & 15 & 1.2e+06 & 4.8e-06 & 7.7  & 15 & 16 & 1.2e+06 & 4.8e-06 \\
3000 & 19.2 & 14 & 15 & 1.7e+06 & 5.0e-06 & 12.7 & 15 & 16 & 1.7e+06 & 5.3e-06 \\
4000 & 44.7 & 14 & 15 & 2.6e+06 & 5.7e-06 & 25.8 & 17 & 18 & 2.6e+06 & 6.1e-06 \\ \hline



==> tab/Test_5_5_1.tex <==
\multirow{4}{*}{GBB}
& 0.01 & 2.0 & 4 & 5 & 9.648e+02 & 4.668e-06 \\
& 0.10 & 2.2 & 6 & 7 & 3.145e+03 & 3.687e-06 \\
& 1.00 & 6.8 & 21 & 22 & 4.472e+04 & 1.656e-07 \\
& 10.00 & 12.2 & 43 & 44 & 5.349e+05 & 8.263e-06 \\ \hline

\multirow{4}{*}{GBB-Inexact}
& 0.01 & 1.8 & 4 & 5 & 9.648e+02 & 4.668e-06 \\
& 0.10 & 2.7 & 6 & 7 & 3.145e+03 & 3.632e-06 \\
& 1.00 & 4.5 & 21 & 22 & 4.472e+04 & 1.515e-07 \\
& 10.00 & 6.3 & 54 & 55 & 5.349e+05 & 7.107e-06 \\ \hline

\multirow{4}{*}{LBFGS}
& 0.01 & 1.1 & 2 & 3 & 9.648e+02 & 9.782e-06 \\
& 0.10 & 1.8 & 5 & 6 & 3.145e+03 & 7.419e-06 \\
& 1.00 & 3.3 & 11 & 12 & 4.472e+04 & 2.049e-06 \\
& 10.00 & 5.8 & 20 & 21 & 5.349e+05 & 2.365e-06 \\ \hline

\multirow{4}{*}{LBFGS-Inexact}
& 0.01 & 1.6 & 2 & 3 & 9.648e+02 & 9.782e-06 \\
& 0.10 & 2.9 & 5 & 6 & 3.145e+03 & 7.220e-06 \\
& 1.00 & 3.2 & 12 & 13 & 4.472e+04 & 9.115e-06 \\
& 10.00 & 4.2 & 23 & 24 & 5.349e+05 & 1.358e-05 \\ \hline

\multirow{4}{*}{Newton}
& 0.01 & 1.2 & 2 & 3 & 9.648e+02 & 1.464e-07 \\
& 0.10 & 2.3 & 4 & 5 & 3.145e+03 & 1.804e-06 \\
& 1.00 & 3.2 & 6 & 7 & 4.472e+04 & 3.210e-06 \\
& 10.00 & 3.8 & 8 & 9 & 5.349e+05 & 3.593e-06 \\ \hline

\multirow{4}{*}{QN-CG}
& 0.01 & 2.9 & 4 & 5 & 9.648e+02 & 2.415e-07 \\
& 0.10 & 3.7 & 8 & 9 & 3.145e+03 & 1.821e-06 \\
& 1.00 & 4.6 & 14 & 16 & 4.472e+04 & 3.269e-06 \\
& 10.00 & 6.2 & 19 & 20 & 5.349e+05 & 3.590e-06 \\ \hline

\multirow{4}{*}{QN-CG-Inexact}
& 0.01 & 4.3 & 4 & 5 & 9.648e+02 & 2.415e-07 \\
& 0.10 & 5.7 & 8 & 9 & 3.145e+03 & 1.822e-06 \\
& 1.00 & 4.2 & 18 & 19 & 4.472e+04 & 3.225e-06 \\
& 10.00 & 4.7 & 27 & 29 & 5.349e+05 & 3.621e-06 \\ \hline

==> tab/Test_5_6_1.tex <==
\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{GBB} & \multicolumn{5}{c|}{IGBB} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 1.0  & 16 & 17 & 8.8e+03 & 2.2e-07 &  0.8  & 16 & 17 & 8.8e+03 & 2.4e-07 \\
1000 & 1.8  & 17 & 18 & 2.6e+04 & 8.7e-06 &  1.3  & 17 & 18 & 2.6e+04 & 1.4e-05 \\
1500 & 5.8  & 19 & 20 & 4.9e+04 & 8.3e-06 &  3.1  & 21 & 22 & 4.9e+04 & 1.5e-05 \\
2000 & 8.9  & 21 & 22 & 7.7e+04 & 9.9e-06 &  5.5  & 22 & 23 & 7.7e+04 & 2.9e-06 \\
2500 & 16.5 & 22 & 23 & 1.1e+05 & 4.5e-07 &  9.1  & 22 & 23 & 1.1e+05 & 1.2e-05 \\
3000 & 27.9 & 22 & 23 & 1.4e+05 & 7.6e-07 &  15.3 & 25 & 26 & 1.4e+05 & 9.0e-06 \\
4000 & 67.8 & 22 & 23 & 2.2e+05 & 1.3e-06 &  33.3 & 26 & 27 & 2.2e+05 & 1.6e-05 \\ \hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{ILBFGS} & \multicolumn{5}{c|}{Newton} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 0.3  & 10 & 11 & 8.8e+03 & 3.7e-06 &  0.5  & 6 & 7 & 8.8e+03 & 1.8e-06 \\
1000 & 0.8  & 11 & 12 & 2.6e+04 & 1.2e-05 &  1.2  & 6 & 7 & 2.6e+04 & 2.6e-06 \\
1500 & 2.2  & 12 & 13 & 4.9e+04 & 9.3e-06 &  2.8  & 6 & 7 & 4.9e+04 & 3.3e-06 \\
2000 & 4.3  & 14 & 15 & 7.7e+04 & 1.6e-06 &  4.7  & 6 & 7 & 7.7e+04 & 3.8e-06 \\
2500 & 8.0  & 14 & 15 & 1.1e+05 & 3.1e-06 &  8.0  & 6 & 7 & 1.1e+05 & 4.3e-06 \\
3000 & 12.1 & 14 & 15 & 1.4e+05 & 2.6e-06 &  13.2 & 6 & 7 & 1.4e+05 & 4.8e-06 \\
4000 & 26.3 & 14 & 15 & 2.2e+05 & 4.8e-06 &  33.2 & 7 & 8 & 2.2e+05 & 5.6e-06 \\ \hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{QN} & \multicolumn{5}{c|}{IQN} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 0.7  & 11 & 12 & 8.8e+03 & 1.7e-06 &  0.5  & 10 & 11 & 8.8e+03 & 1.8e-06 \\
1000 & 1.4  & 11 & 12 & 2.6e+04 & 2.8e-06 &  1.2  & 10 & 11 & 2.6e+04 & 2.5e-06 \\
1500 & 3.7  & 12 & 13 & 4.9e+04 & 3.1e-06 &  3.1  & 11 & 12 & 4.9e+04 & 3.2e-06 \\
2000 & 5.5  & 11 & 12 & 7.7e+04 & 4.1e-06 &  4.8  & 11 & 12 & 7.7e+04 & 3.7e-06 \\
2500 & 10.6 & 12 & 13 & 1.1e+05 & 4.4e-06 &  8.8  & 11 & 12 & 1.1e+05 & 4.3e-06 \\
3000 & 17.3 & 12 & 13 & 1.4e+05 & 4.9e-06 &  13.1 & 11 & 12 & 1.4e+05 & 4.8e-06 \\
4000 & 39.8 & 12 & 13 & 2.2e+05 & 5.9e-06 &  27.4 & 12 & 13 & 2.2e+05 & 5.6e-06 \\ \hline



==> tab/Test_5_7.tex <==
\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{GBB} & \multicolumn{5}{c|}{IGBB} \ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$& time & iter & feval & $f$ & $\|g\|$ \\ \hline
  500 &    1.1 &   33 &   34 & 1.3e+05 & 1.0e-05 &    0.9 &   43 &   44 & 1.3e+05 & 1.2e-06 \\ 
 1000 &    3.8 &   43 &   44 & 5.0e+05 & 5.4e-06 &    1.4 &   54 &   55 & 5.0e+05 & 4.5e-06 \\ 
 1500 &   12.3 &   54 &   55 & 1.1e+06 & 5.6e-06 &    3.3 &   68 &   69 & 1.1e+06 & 9.8e-06 \\ 
 2000 &   25.0 &   65 &   66 & 2.0e+06 & 3.5e-06 &    5.8 &   79 &   80 & 2.0e+06 & 9.8e-06 \\ 
 2500 &   66.4 &   98 &   99 & 3.1e+06 & 4.8e-06 &   12.6 &  131 &  132 & 3.1e+06 & 6.0e-06 \\ 
 3000 &  119.6 &  102 &  103 & 4.5e+06 & 9.8e-06 &   21.2 &  142 &  143 & 4.5e+06 & 9.8e-06 \\ 
 4000 &  341.8 &  120 &  121 & 8.0e+06 & 8.1e-06 &   49.0 &  186 &  187 & 8.0e+06 & 1.2e-05 \\ 
\hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{ILBFGS} & \multicolumn{5}{c|}{Newton} \ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$& time & iter & feval & $f$ & $\|g\|$ \\ \hline
  500 &    0.4 &   31 &   32 & 1.3e+05 & 4.8e-06 &    0.7 &    9 &   10 & 1.3e+05 & 2.2e-06 \\ 
 1000 &    0.8 &   31 &   32 & 5.0e+05 & 9.0e-06 &    1.6 &    9 &   10 & 5.0e+05 & 3.1e-06 \\ 
 1500 &    2.1 &   36 &   37 & 1.1e+06 & 8.2e-06 &    4.1 &   10 &   11 & 1.1e+06 & 3.8e-06 \\ 
 2000 &    4.3 &   37 &   38 & 2.0e+06 & 8.6e-06 &    7.3 &   10 &   11 & 2.0e+06 & 4.4e-06 \\ 
 2500 &    7.5 &   39 &   40 & 3.1e+06 & 1.1e-05 &   12.3 &   10 &   11 & 3.1e+06 & 4.9e-06 \\ 
 3000 &   12.1 &   39 &   41 & 4.5e+06 & 8.1e-06 &   20.8 &   10 &   11 & 4.5e+06 & 5.4e-06 \\ 
 4000 &   25.0 &   44 &   45 & 8.0e+06 & 1.1e-05 &   48.3 &   11 &   12 & 8.0e+06 & 6.3e-06 \\ 
\hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{QN} & \multicolumn{5}{c|}{IQN} \ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$& time & iter & feval & $f$ & $\|g\|$ \\ \hline
  500 &    0.8 &   20 &   21 & 1.3e+05 & 2.1e-06 &    0.5 &   20 &   21 & 1.3e+05 & 2.2e-06 \\ 
 1000 &    2.3 &   22 &   23 & 5.0e+05 & 3.1e-06 &    1.4 &   22 &   23 & 5.0e+05 & 3.2e-06 \\ 
 1500 &    6.0 &   24 &   25 & 1.1e+06 & 3.8e-06 &    2.5 &   22 &   23 & 1.1e+06 & 3.8e-06 \\ 
 2000 &   10.9 &   25 &   26 & 2.0e+06 & 4.4e-06 &    4.5 &   24 &   25 & 2.0e+06 & 4.4e-06 \\ 
 2500 &   20.0 &   25 &   26 & 3.1e+06 & 4.9e-06 &    7.6 &   24 &   25 & 3.1e+06 & 4.9e-06 \\ 
 3000 &   33.1 &   26 &   27 & 4.5e+06 & 5.4e-06 &   13.1 &   24 &   25 & 4.5e+06 & 5.4e-06 \\ 
 4000 &   78.6 &   26 &   27 & 8.0e+06 & 6.2e-06 &   31.4 &   24 &   25 & 8.0e+06 & 6.3e-06 \\ 
\hline



==> tab/Test_5_7_1.tex <==
\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{GBB} & \multicolumn{5}{c|}{IGBB} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 1.1   & 33  & 34  & 1.2e+05 & 9.9e-06 & 0.6  & 43  & 44  & 1.2e+05 & 1.1e-06 \\
1000 & 3.6   & 44  & 45  & 5.0e+05 & 8.7e-06 & 1.7  & 54  & 55  & 5.0e+05 & 5.4e-06 \\
1500 & 11.3  & 54  & 55  & 1.1e+06 & 7.0e-06 & 3.3  & 68  & 69  & 1.1e+06 & 9.4e-06 \\
2000 & 25.0  & 65  & 66  & 2.0e+06 & 2.4e-06 & 5.7  & 81  & 82  & 2.0e+06 & 1.0e-05 \\
2500 & 65.8  & 98  & 99  & 3.1e+06 & 6.1e-06 & 13.5 & 130 & 131 & 3.1e+06 & 9.8e-06 \\
3000 & 127.6 & 109 & 110 & 4.5e+06 & 5.7e-06 & 23.0 & 148 & 149 & 4.5e+06 & 1.0e-05 \\
4000 & 342.1 & 120 & 121 & 8.0e+06 & 6.4e-06 & 47.7 & 175 & 176 & 8.0e+06 & 1.0e-05 \\ \hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{ILBFGS} & \multicolumn{5}{c|}{Newton} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
500  & 0.5  & 32 & 34 & 1.2e+05 & 7.5e-06 & 0.5  & 9  & 10 & 1.2e+05 & 2.1e-06 \\
1000 & 1.3  & 37 & 39 & 5.0e+05 & 6.2e-06 & 1.7  & 9  & 10 & 5.0e+05 & 3.0e-06 \\
1500 & 2.1  & 39 & 40 & 1.1e+06 & 5.8e-06 & 4.2  & 10 & 11 & 1.1e+06 & 3.7e-06 \\
2000 & 4.6  & 43 & 45 & 2.0e+06 & 3.0e-06 & 7.2  & 10 & 11 & 2.0e+06 & 4.3e-06 \\
2500 & 8.8  & 45 & 48 & 3.1e+06 & 8.7e-06 & 12.2 & 10 & 11 & 3.1e+06 & 4.9e-06 \\
3000 & 15.7 & 47 & 52 & 4.5e+06 & 9.1e-06 & 20.8 & 10 & 11 & 4.5e+06 & 5.4e-06 \\
4000 & 27.6 & 49 & 52 & 8.0e+06 & 8.4e-06 & 48.6 & 11 & 12 & 8.0e+06 & 6.2e-06 \\ \hline

\multirow{2}{*}{$n$} & \multicolumn{5}{c|}{QN} & \multicolumn{5}{c|}{IQN} \\ \cline{2-11}
& time & iter & feval & $f$ & $\|g\|$ & time & iter & feval & $f$ & $\|g\|$ \\ \hline
  500 &    0.8 &   20 &   21 & 1.3e+05 & 2.1e-06 & 0.6  & 21 & 22 & 1.2e+05 & 2.1e-06 \\
 1000 &    2.3 &   22 &   23 & 5.0e+05 & 3.1e-06 & 1.3  & 21 & 22 & 5.0e+05 & 3.1e-06 \\
 1500 &    6.0 &   24 &   25 & 1.1e+06 & 3.8e-06 & 2.3  & 22 & 23 & 1.1e+06 & 3.8e-06 \\
 2000 &   10.9 &   25 &   26 & 2.0e+06 & 4.4e-06 & 4.2  & 23 & 24 & 2.0e+06 & 4.4e-06 \\
 2500 &   20.0 &   25 &   26 & 3.1e+06 & 4.9e-06 & 7.2  & 24 & 25 & 3.1e+06 & 4.9e-06 \\
 3000 &   33.1 &   26 &   27 & 4.5e+06 & 5.4e-06 & 10.5 & 25 & 26 & 4.5e+06 & 5.4e-06 \\
 4000 &   78.6 &   26 &   27 & 8.0e+06 & 6.2e-06 & 24.8 & 24 & 25 & 8.0e+06 & 6.3e-06 \\ \hline



==> tab/ncm.tex <==
\multicolumn{13}{c}{Results of Example \ref{eg:5.5}} \\ \hline
\multirow{2}{*}{$n$} & \multicolumn{4}{c|}{GBB} & \multicolumn{4}{c|}{IGBB} & \multicolumn{4}{c|}{Newton} \\ \cline{2-13}
& time & iter & $f$ & $\|g\|$ & time & iter & $f$ & $\|g\|$ & time & iter & $f$ & $\|g\|$ \\ \hline
500  & 0.9   & 43 & 1.1e+05 & 4.6e-06 & 0.4  & 47 & 1.1e+05 & 9.9e-06 & 0.5  & 8 & 1.1e+05 & 2.1e-06 \\
1000 & 3.6   & 43 & 3.1e+05 & 6.9e-06 & 1.6  & 54 & 3.1e+05 & 4.6e-06 & 1.3  & 8 & 3.1e+05 & 3.0e-06 \\
1500 & 9.4   & 43 & 5.9e+05 & 9.2e-06 & 3.6  & 56 & 5.9e+05 & 9.9e-06 & 3.3  & 8 & 5.9e+05 & 3.7e-06 \\
2000 & 19.0  & 50 & 9.2e+05 & 9.9e-06 & 5.6  & 65 & 9.2e+05 & 3.7e-06 & 6.0  & 8 & 9.2e+05 & 4.3e-06 \\
2500 & 37.4  & 54 & 1.2e+06 & 1.0e-06 & 9.8  & 65 & 1.2e+06 & 4.1e-06 & 10.0 & 8 & 1.2e+06 & 4.8e-06 \\
3000 & 64.3  & 54 & 1.7e+06 & 1.1e-06 & 16.0 & 65 & 1.7e+06 & 5.2e-06 & 16.7 & 8 & 1.7e+06 & 5.3e-06 \\
4000 & 155.2 & 54 & 2.6e+06 & 1.3e-06 & 35.3 & 76 & 2.6e+06 & 4.2e-06 & 36.2 & 8 & 2.6e+06 & 6.1e-06 \\ \hline \hline

\multicolumn{13}{c}{Results of Example \ref{eg:5.6}} \\ \hline
\multirow{2}{*}{$n$} & \multicolumn{4}{c|}{GBB} & \multicolumn{4}{c|}{IGBB} & \multicolumn{4}{c|}{Newton} \\ \cline{2-13}
& time & iter & $f$ & $\|g\|$ & time & iter & $f$ & $\|g\|$ & time & iter & $f$ & $\|g\|$ \\ \hline
500  & 1.0  & 16 & 8.8e+03 & 2.2e-07 &  0.8  & 16 & 8.8e+03 & 2.4e-07 & 0.5  & 6 & 8.8e+03 & 1.8e-06\\
1000 & 1.8  & 17 & 2.6e+04 & 8.7e-06 &  1.3  & 17 & 2.6e+04 & 1.4e-05 & 1.2  & 6 & 2.6e+04 & 2.6e-06\\
1500 & 5.8  & 19 & 4.9e+04 & 8.3e-06 &  3.1  & 21 & 4.9e+04 & 1.5e-05 & 2.8  & 6 & 4.9e+04 & 3.3e-06\\
2000 & 8.9  & 21 & 7.7e+04 & 9.9e-06 &  5.5  & 22 & 7.7e+04 & 2.9e-06 & 4.7  & 6 & 7.7e+04 & 3.8e-06\\
2500 & 16.5 & 22 & 1.1e+05 & 4.5e-07 &  9.1  & 22 & 1.1e+05 & 1.2e-05 & 8.0  & 6 & 1.1e+05 & 4.3e-06\\
3000 & 27.9 & 22 & 1.4e+05 & 7.6e-07 &  15.3 & 25 & 1.4e+05 & 9.0e-06 & 13.2 & 6 & 1.4e+05 & 4.8e-06\\
4000 & 67.8 & 22 & 2.2e+05 & 1.3e-06 &  33.3 & 26 & 2.2e+05 & 1.6e-05 & 33.2 & 7 & 2.2e+05 & 5.6e-06\\ \hline \hline

\multicolumn{13}{c}{Results of Example \ref{eg:5.7}} \\ \hline
\multirow{2}{*}{$n$} & \multicolumn{4}{c|}{GBB} & \multicolumn{4}{c|}{IGBB} & \multicolumn{4}{c|}{Newton} \\ \cline{2-13}
& time & iter & $f$ & $\|g\|$ & time & iter & $f$ & $\|g\|$ & time & iter & $f$ & $\|g\|$ \\ \hline
500  & 1.1   & 33  & 1.2e+05 & 9.9e-06 & 0.6  & 43  & 1.2e+05 & 1.1e-06 & 0.5  & 9  & 1.2e+05 & 2.1e-06 \\
1000 & 3.6   & 44  & 5.0e+05 & 8.7e-06 & 1.7  & 54  & 5.0e+05 & 5.4e-06 & 1.7  & 9  & 5.0e+05 & 3.0e-06 \\
1500 & 11.3  & 54  & 1.1e+06 & 7.0e-06 & 3.3  & 68  & 1.1e+06 & 9.4e-06 & 4.2  & 10 & 1.1e+06 & 3.7e-06 \\
2000 & 25.0  & 65  & 2.0e+06 & 2.4e-06 & 5.7  & 81  & 2.0e+06 & 1.0e-05 & 7.2  & 10 & 2.0e+06 & 4.3e-06 \\
2500 & 65.8  & 98  & 3.1e+06 & 6.1e-06 & 13.5 & 130 & 3.1e+06 & 9.8e-06 & 12.2 & 10 & 3.1e+06 & 4.9e-06 \\
3000 & 127.6 & 109 & 4.5e+06 & 5.7e-06 & 23.0 & 148 & 4.5e+06 & 1.0e-05 & 20.8 & 10 & 4.5e+06 & 5.4e-06 \\
4000 & 342.1 & 120 & 8.0e+06 & 6.4e-06 & 47.7 & 175 & 8.0e+06 & 1.0e-05 & 48.6 & 11 & 8.0e+06 & 6.2e-06 \\ \hline


